Structured Video Tokens @ Ego4D PNR Temporal Localization Challenge 2022

This technical report describes the SViT approach for the Ego4D Point of No Return (PNR) Temporal Localization Challenge. We propose a learning framework StructureViT (SViT for short), which demonstrates how utilizing the structure of a small number of images only available during training can improve a video model. SViT relies on two key insights. First, as both images and videos contain structured information, we enrich a transformer model with a set of \emph{object tokens} that can be used across images and videos. Second, the scene representations of individual frames in video should "align" with those of still images. This is achieved via a "Frame-Clip Consistency" loss, which ensures the flow of structured information between images and videos. SViT obtains strong performance on the challenge test set with 0.656 absolute temporal localization error.

==> Tables/Experiments/ego4d_ood.tex <==
\begin{tabularx}
{1\linewidth}{@{}l c c c}
        \toprule
         Image Data & Top 1 & Loc. Error \\
        \midrule
        100DOH+Ego4d & - & - \\
        100DOH & - & - \\
        \bottomrule
\end{tabularx}


==> Tables/Experiments/smthelse_Relations_part.tex <==
\begin{tabularx}
{0.8\linewidth}{@{}l c c}
        \toprule


         Model & Top-1 \\
        \midrule
        SViT -Contact &  65.5 \\
%%        None & 65.3  \\
        SViT -Contact -Corresp. & 65.3  \\
%%        +Object Tokens (OT) Cor. &  65.5 \\
%%        +OT Cor. + Contact (SViT) & 65.8  \\
%%        +OT Cor. + Contact + Geo. & 65.7 \\
        SViT +Geometry & 65.7 \\
                SViT & 65.8  \\
        \bottomrule
\end{tabularx}


==> Tables/Experiments/smthelse_ablation_consistency.tex <==
\begin{table}[t!]
  \scriptsize
%   \tablestyle{2.0pt}{1.00}
   \centering
    \begin{tabular}{l c c}
            \toprule
             Model & Top-1 \\
            \midrule
            No consistency & 65  \\
            +Patch Tokens consistency & - \\
            +EgoGraph consistency & 65.3  \\
            +EgoGraph consistency +Object Tokens consistency & 65.6  \\
            \bottomrule
   \end{tabular}%
    \caption{\textbf{Consistency loss ablation} on the ``SmthElse'' dataset.
  }
  % Results of Point-of-no-return temporal localization error (seconds)
    \label{tab:comp_fewshot}
\end{table}


==> Tables/Experiments/smthelse_ablation_tokens_consistency.tex <==
\begin{table}[t!]
  \scriptsize
%   \tablestyle{2.0pt}{1.00}
   \centering
    \begin{tabular}{l c c}
            \toprule
             Model & Top-1 \\
            \midrule
            MViT & 63.3  \\
            MViT-multitask & 63.8  \\
            MViT +Object Tokens & 65.0  \\
            MViT +Object Tokens +Consistency (Ours) & 65.6  \\
            \bottomrule
   \end{tabular}%
    \caption{\textbf{Method components ablation} on the ``SmthElse'' dataset.
  }
  % Results of Point-of-no-return temporal localization error (seconds)
    \label{tab:comp_fewshot}
\end{table}


==> Tables/Experiments/smthelse_ablation_tokens_consistency_part.tex <==
\begin{tabularx}
{1\linewidth}{@{}l c c@{}}
        \toprule
         Model & Top-1 \\
        \midrule
        MViTv2 & 63.3  \\
        MViTv2 MT & 63.8  \\
        MViTv2 +Object Tokens (OT) & 65.0  \\
        MViTv2 +OT +FC Loss (\model) & 65.8  \\
        \bottomrule
\end{tabularx}


==> Tables/Experiments/smthelse_data_ratio.tex <==
\begin{table}[t!]
  \scriptsize
%   \tablestyle{2.0pt}{1.00}
   \centering
    \begin{tabular}{l c c}
            \toprule


             $\%$ of data & Top-1 \\
            \midrule
            0 & 65.1 \\
            2 & 65.6  \\
            25 & 65.6  \\
            50 & 65.7  \\
            100 & 65.8  \\
            \bottomrule
    \end{tabular}%
    \caption{\textbf{$\%$ of data} on the ``SmthElse'' dataset.
  }
  % Results of Point-of-no-return temporal localization error (seconds)
    \label{tab:comp_fewshot}
\end{table}

==> Tables/Experiments/smthelse_data_ratio_part.tex <==
% \newcommand{\rowspace}{\vspace{0.15cm}}
\newcommand{\rowspace}{}

\begin{tabularx}
{1\linewidth}{@{}l c c}
        \toprule


         $\%$ of data & Top-1 \\
        \midrule
        \rowspace
        % 0 &  \\
        2 & 65.6  \\
        \rowspace
        25 & 65.6  \\
        \rowspace
        50 & 65.7  \\
        \rowspace
        100 & 65.8  \\
        \bottomrule
\end{tabularx}


==> Tables/Experiments/smthelse_det_part.tex <==
\begin{tabularx}
{1\linewidth}{@{}l c c}
        \toprule
         Model & mAP \\
        \midrule
        Det. only & 0.158  \\
        SS2V & 0.155  \\
        \bottomrule
\end{tabularx}


==> Tables/Experiments/smthelse_predFromGraph_part.tex <==
\begin{tabularx}
{1\linewidth}{@{}l c c}
        \toprule
         Model & Top1 \\
        \midrule
        SS2V & 63.8  \\
        SS2V /w & \\
        HAOG & -  \\
        \bottomrule
\end{tabularx}


==> Tables/Experiments/smthelse_tokensCons_dataRatio_combined.tex <==
\begin{table*}[t]
    % components
    % \footnotesize
    \begin{subtable}[t]{0.35\textwidth}
    \tablestyle{1.0pt}{1.00}
        \caption{{Method components}}
        \input{Tables/Experiments/smthelse_ablation_tokens_consistency_part}
        \label{tab:abl_components}
    \end{subtable}
    %  \hspace
    \hfill
    \begin{subtable}[t]{0.18\linewidth}
    \tablestyle{6.0pt}{1.00}
        \caption{{Images Amount}}
        \input{Tables/Experiments/smthelse_data_ratio_part}
        \label{tab:abl_data_ratio}
     \end{subtable}
    %  \hspace{0.2cm}
    % \hfill
    \begin{subtable}[t]{0.40\textwidth}
    \tablestyle{4.0pt}{1.00}
        % \vspace{3cm}
        \centering
        \caption{{{\graph} Attributes}}
        \input{Tables/Experiments/smthelse_Relations_part}
        \label{tab:abl_relations}
     \end{subtable}
     \caption{\textbf{Ablations.} We show (a) Contributions of {\approach} components. (b) Amount of annotated images used in training. (c) Examine different {\graph} information. The experiments are performed on the SomethingElse split. For more ablations, see supplementary.}
     \label{tab:ablations}
     \vspace{-10pt}
\end{table*}




    %  \hspace{0.2cm}
    % det
    % \begin{subtable}[t]{0.185\textwidth}
    %     % \vspace{3cm}
    %     \caption{\textbf{Detections}}
    %     \input{Tables/Experiments/smthelse_det_part}
    %     \label{tab:abl_det}
    %  \end{subtable}
    % % ego4d ood
    % \begin{subtable}{0.4\textwidth}
    %     % \vspace{3cm}
    %     \caption{\textbf{Ego4D Image Source}}
    %     \input{Tables/Experiments/ego4d_ood}
    %     \label{tab:abl_data_ratio}
    %  \end{subtable}
    % pred from graph
    % \begin{subtable}[t]{0.17\textwidth}
    %     % \vspace{3cm}
    %     \caption{\textbf{Use HAOG}}
    %     \input{Tables/Experiments/smthelse_predFromGraph_part}
    %     \label{tab:abl_pred_from_graph}
    %  \end{subtable}

==> Tables/Results/diving48.tex <==
\begin{tabularx}
{\linewidth}{@{}l c r@{} r}
    \toprule
    {Model} & Frames & {Top-1} \\ 
    \midrule
    I3D & 8 & 48.3 \\
    TSM & 3 & 51.1 \\
    TSN & 3 & 52.5 \\
    % TRNms & ImageNet & 3 & 66.0\\
    GST-50 & 8 & 78.9 \\
    ST-S3D & 8 & 50.6 \\
    \midrule
    SlowFast, R101 & 16 & 77.6 \\
    TimeSformer & 16 & 74.9 \\
    TimeSformer-HR & 16 & 78.0 \\
    % TimeSformer-L & 96 & 81.0 \\
    MViTv2-S & 16 & 73.1 \\

    \midrule
    {\model} - & & \\
    Standard Finetune & 16 & TODO \\
    {\model} & 16 & 79.8 \\

    \bottomrule
\end{tabularx}


==> Tables/Results/diving48_noFrames.tex <==
\renewcommand*{\thefootnote}{\fnsymbol{footnote}}
\begin{tabularx}
{\linewidth}{@{}l l c c}
    \toprule
    {Model} & {Top-1} \\ 
    & \\ 
    % \midrule
    % I3D  & 48.3 \\
    % TSM  & 51.1 \\
    % TSN  & 52.5 \\
    % % TRNms & ImageNet & 3 & 66.0\\
    % GST-50  & 78.9 \\
    % ST-S3D  & 50.6 \\
    \midrule
    SlowFast, R101 \methodwithoutboxes & 77.6 \\
    TimeSformer \methodwithoutboxes & 74.9 \\
    TimeSformer-HR \methodwithoutboxes & 78.0 \\
    % TimeSformer-L & 96 & 81.0 \\
    MViTv2 \methodwithoutboxes  & 73.1 \\
    \midrule
    {MViTv2 MT} & 75.5 \\ % no consistecy, no obj tok
    \midrule
    {\modelPT}  & 77.9\gcol{$+$4.8} \\
    {\modelDD}  & 79.8\gcol{$+$6.7} \\
    \bottomrule
\end{tabularx}


==> Tables/Results/ego4d_pnr_classification.tex <==
\begin{table}[t!]
  \scriptsize
%   \tablestyle{2.0pt}{1.00}
   \centering
    \begin{tabular}{l c c}
            \toprule


             Model & Accuracy  \\
            \midrule
            {Bi-directional LSTM} & 65.3  \\
            {I3D ResNet-50} & 68.7  \\
            {MViT-v2} & -  \\
            \midrule
            {Ours} & -  \\
            \bottomrule
   \end{tabular}%
    \caption{\textbf{Point-of-no-return classification} on the ``Ego4d'' dataset.
  }
  % Results of Point-of-no-return temporal localization error (seconds)
    \label{tab:comp_fewshot}
\end{table}


==> Tables/Results/ego4d_pnr_cls_part.tex <==
\begin{tabularx}
{0.8\linewidth}{@{}l c c}
            \toprule
             Model & Accuracy  \\
            \midrule
            {Bi-directional LSTM} & 65.3  \\
            {I3D ResNet-50} & 68.7  \\
            {MViT-v2} & -  \\
            \midrule
            {Ours} & -  \\
            \bottomrule
    \label{tab:comp_fewshot}
\end{tabularx}


==> Tables/Results/ego4d_pnr_localization.tex <==
\begin{table}[t!]
  \scriptsize
%   \tablestyle{2.0pt}{1.00}
   \centering
    \begin{tabular}{l c c}
            \toprule


             Model & localization error \\ & (seconds)  \\
            \midrule
            {BMN} & 0.780  \\
            {I3D ResNet-50} & 0.739  \\
            {Bi-directional LSTM} & 0.790  \\
            {MViT-v2} & -  \\
            \midrule
            {Ours} & 0.515  \\
            \bottomrule
   \end{tabular}%
    \caption{\textbf{Point-of-no-return temporal localization} on the ``Ego4d'' dataset.
  }
  % Results of Point-of-no-return temporal localization error (seconds)
    \label{tab:comp_fewshot}
\end{table}


==> Tables/Results/ego4d_unified.tex <==
\begin{table}[t!]
  \scriptsize
%   \tablestyle{2.0pt}{1.00}
   \centering
    \begin{tabular}{l c c c}
            \toprule


             Model & Temporal localization & Classification\\ & error (seconds) & accuracy  \\
            \midrule
            {Bi-directional LSTM} & 0.790  & 65.3 \\
            {BMN}                 & 0.780  & - \\
            {I3D ResNet-50}       & 0.739  & 68.7 \\
            {MViT-v2}             & 0.702  & 71.6 \\
            \midrule
            {Ours}                & 0.515  & 73.8 \\
            \bottomrule
   \end{tabular}%
    \caption{\textbf{Point-of-no-return temporal localization and classification} on the ``Ego4d'' dataset.
  }
  % Results of Point-of-no-return temporal localization error (seconds)
    \label{tab:comp_fewshot}
\end{table}


==> Tables/Results/ego4d_unified_part.tex <==
\renewcommand*{\thefootnote}{\fnsymbol{footnote}}
% \newcommand{\rowspace}{\vspace{0.0375cm}}
\newcommand{\rowspace}{}
\begin{tabularx}
{1\linewidth}{@{}l c c c c c c}
            \toprule
             Model & Pretraining & Finetuning  & Object & Frame-Clip & Val Temporal & Test Temporal  \\
                   & Aux. Images & Aux. Images & Tokens & Consistency Loss & loc. error   & loc. error \\
            \midrule
            {Bi-LSTM} \methodwithoutboxes & - & - & \xmark & \xmark & 0.790 &  - \\
            \rowspace
            {BMN}\methodwithoutboxes    & - & - & \xmark & \xmark & 0.780 &  \\
            \rowspace
            {I3D ResNet-50}\methodwithoutboxes   & - & - & \xmark & \xmark & 0.739 & \\
            \rowspace
            {MViT-v2}\methodwithoutboxes   & - & - & \xmark & \xmark & 0.702 & \\
            \midrule
            	
            {MViTv2 MT} & Ego4D, 100DOH & Ego4D, 100DOH & \xmark & \xmark & 0.595 & \\ % no consistecy, no obj tok
            \midrule

            {\modelPT} & Ego4D, 100DOH & - & \cmark & \cmark & 0.544 &  \\ % "multi task" pretrain
            \rowspace
            {\modelDD} & 100DOH & 100DOH & \cmark & \cmark & 0.527 & \\
            \rowspace
            {{\modelID}} & Ego4D, 100DOH & Ego4D & \cmark & \cmark & 0.515 & \\
            \bottomrule
\end{tabularx}

==> Tables/Results/results_ego4d_ssv2_combined.tex <==
\renewcommand*{\thefootnote}{\fnsymbol{footnote}}
\begin{table*}[tb!]
    \begin{subtable}[t]{0.37\textwidth}
        \tablestyle{4.0pt}{1.00}
    	\centering
        % \caption{{Object State Change in Ego4D}.}
        \input{Tables/Results/ego4d_unified_part}
        \label{tab:ego4d}
     \end{subtable}
    \caption{\textbf{Results on Ego4D PNR Temporal Localization.} {We denote methods that do not use any additional structured annotation with \protect\methodwithoutboxes}.}
    \label{tab:temps}
    \vspace{-10pt}
\end{table*}







==> Tables/Results/smthelse.tex <==
\begin{table}[t!]
%   \scriptsize
%   \tablestyle{2.0pt}{1.00}
   \centering
    \begin{tabular}{l cc cc cc cc cc}
            \toprule

            \multirow{2}{*}{Model} & \multicolumn{2}{c}{Boxes} & \multicolumn{2}{c}{Compositional} & \multicolumn{2}{c}{Base} & \multicolumn{2}{c}{Few-Shot} \\ 

             & Input & Supervision & {Top-1} & {Top-5} & {Top-1} & {Top-5} & {5-Shot} & {10-Shot}  \\
            
            % \cmidrule(l{0pt}r{0pt}){2-3} 
            \midrule
            {I3D~\cite{carreira2017quo}} & \xmark & \xmark & 42.8 & 71.3 & 73.6 & 92.2 & 21.8 & 26.7 \\
            {SlowFast~\cite{slowfast2019}} & \xmark & \xmark & 45.2 & 73.4 & 76.1 & 93.4 & 22.4 & 29.2 \\
            {TimeSformer~\cite{gberta_2021_ICML}} & \xmark & \xmark &  44.2 & 76.8 & 79.5 & 95.6 & 24.6 & 33.8 \\
            {Mformer~\cite{patrick2021keeping}} & \xmark & \xmark &   60.2 & 85.8 & 82.8 & 96.2 & 28.9 & 33.8 \\
            {MViT~\cite{}} & \xmark & \xmark &  63.3 & 87.5 & 83.7 & 96.8 & - & - \\

            % \midrule

            % {STRG (\textbackslash{w}~SF)~\cite{Wang_videogcnECCV2018}} &  \cmark & \xmark &   52.3 & 78.3 & 75.4 & 92.7 & 24.8 & 29.9 \\
            % {STIN} (\textbackslash{w}~SF)~\cite{materzynska2019something} & \cmark & \xmark &   54.6 & 79.4 & 77.4 & 95.0 & 23.0 & 33.4 \\
            % {Mformer+STRG+STIN} & \cmark & \xmark &   62.3 & 86.0 & 83.7 & 96.8 & 29.8 & 36.5 \\
            % {ORViT~Mformer} & \cmark & \xmark &  69.7 & 91.0 & 87.1 & 97.6 & 33.3 & 40.2 \\

            \midrule
            % {MViT+Video Graphs} & \cmark & 65.8 & - & 84.7 & 97.3 & - & - \\
            {MViT multi-task} & \xmark & \cmark &  63.8 & 87.3 & - & - & - & - \\ % no consistecy, no obj tok
            {MViT pretrain} & \xmark & \cmark &  - & - & - & - & - & - \\ % "multi task" pretrain

            \midrule
            {Ours- Non-overlapping} & \xmark & \cmark &  65.1 & 88.0 & - & - & - & - \\
            {Ours- Semi-Supervised $\times 2\%$} & \xmark & \cmark &  65.6 & 88.1 & - & - & - & - \\
            {Ours} & \xmark & \cmark &  65.8 & 88.3 & - & - & - & - \\
            \bottomrule
   \end{tabular}%
    \caption{\textbf{Compositional and Few-Shot Action Recognition} on the ``SomethingElse'' dataset.
  }
    \label{tab:comp_fewshot}
\end{table}


==> Tables/Results/smthelse_no_orvit.tex <==
\begin{table}[t!]
%   \scriptsize
%   \tablestyle{1.0pt}{1.00}
   \centering
    \begin{tabular}{l cc cc cc cc cc}
            \toprule

            \multirow{2}{*}{Model} & {Boxes} & \multicolumn{2}{c}{Compositional} & \multicolumn{2}{c}{Base} & \multicolumn{2}{c}{Few-Shot} \\ 

             & Annotations & {Top-1} & {Top-5} & {Top-1} & {Top-5} & {5-Shot} & {10-Shot}  \\
            \midrule
            % {I3D~\cite{carreira2017quo}} & \xmark & 42.8 & 71.3 & 73.6 & 92.2 & 21.8 & 26.7 \\
            {SlowFast~\cite{slowfast2019}} & \xmark & 45.2 & 73.4 & 76.1 & 93.4 & 22.4 & 29.2 \\
            {TimeSformer~\cite{gberta_2021_ICML}} & \xmark &  44.2 & 76.8 & 79.5 & 95.6 & 24.6 & 33.8 \\
            {Mformer~\cite{patrick2021keeping}} & \xmark  &   60.2 & 85.8 & 82.8 & 96.2 & 28.9 & 33.8 \\
            {MViTv2~\cite{li2021improvedmvit}} & \xmark &  63.3 & 87.5 & 83.7 & 96.8 & 32.7 & 40.2 \\


            \midrule
            % {MViT+Video Graphs} & \cmark & 65.8 & - & 84.7 & 97.3 & - & - \\
            {MViTv2 MT} & \cmark  &  63.8 & 87.3 & 85.2 & 97.1 & 33.7 & 41.4 \\

            \midrule
            {\modelPT} & \cmark    &  64.2 & 87.9 & 85.0 & 97.1 & 33.8 & 41.7 \\ % "multi task" pretrain
            {\modelDD} & \cmark &  65.1 & 88.0 & 85.8 & 97.4 & 34.6 & 42.5 \\
            {{\model} $\times 2\%$} & \cmark &  65.6 & 88.1 & 85.9 & 97.4 & 34.4 & 43.1 \\
            {\modelID} & \cmark &  65.8 & 88.3 & 85.6 & 97.3 & 34.4 & 42.6 \\
            \bottomrule
   \end{tabular}%
    \caption{\textbf{Compositional and Few-Shot Action Recognition} on the ``SomethingElse'' dataset.
  }
    \label{tab:comp_fewshot}
\end{table}


==> Tables/Results/ssv2.tex <==
\begin{table}[t!]
  \scriptsize
%   \tablestyle{2.0pt}{1.00}
   \centering
    \begin{tabular}{l c c c}
            \toprule


             Model & {Top-1} & {Top-5}  \\
            \midrule
            SlowFast, R101              & 63.1 & 87.6  \\
            TimeSformer-L               & 62.5 & - \\
            ViViT-L                     & 65.4 & 89.8 \\
            MViTv1-B, 16 $\times$ 4     &  64.7 &  89.2 \\
            MViTv2-S, 16 $\times$ 4     &  68.2 &  91.4 \\
            \midrule
            {MViT multi task}           & - & - \\ % no consistecy, no obj tok
            {MViT pretrain}             & - & - \\ % "multi task" pretrain
            \midrule
            {Ours- Non-overlapping}     & -  & - \\ % Running
            {Ours}                      & -  & - \\ % Running
            \bottomrule
   \end{tabular}%
    \caption{\textbf{Action Recognition} on the ``SSv2'' dataset.
  }
  % Results of Point-of-no-return temporal localization error (seconds)
    \label{tab:comp_fewshot}
\end{table}

% \renewcommand*{\thefootnote}{\fnsymbol{footnote}}
% \begin{tabularx}
% {0.9\linewidth}{@{}l c c c c r@{}}
%     \toprule
%     {Model} & Boxes & Pretrain & {Top-1} & {Top-5}\\ 
%     \midrule
%     % SlowFast, R50 & \xmark & K400 & 61.7 & 87.0 & 65.7$\times$3$\times$1 & 34.1 \\
%     SlowFast, R101 & \xmark & K400 & 63.1 & 87.6  \\
%     TimeSformer-L & \xmark & IN & 62.5 & - \\
%     ViViT-L & \xmark & {\scriptsize IN+K400}  & 65.4 & 89.8 \\
%     MViT-B, 64 & \xmark & K600  &  68.7 &  91.5 \\

%     \midrule
    

%     \midrule
    

%     \bottomrule
% \end{tabularx}



==> Tables/Results/ssv2_part.tex <==
% \newcommand{\rowspace}{\vspace{0.075cm}}
\newcommand{\rowspace}{}

\begin{tabularx}
{1\linewidth}{@{}l c c c}
            \toprule
             Model & {Top-1} & {Top-5}  \\
             & & & \\
            \midrule
            SlowFast, R101              & 63.1 & 87.6  \\
            \rowspace
            % TimeSformer-L               & 62.5 & - \\
            ViViT-L                     & 65.4 & 89.8 \\
            \rowspace
            MViTv1-B, 16 $\times$ 4     &  64.7 &  89.2 \\
            \rowspace
            MViTv2-S, 16 $\times$ 4     &  68.1 &  90.7 \\
            \midrule
            {MViTv2 multi-task}           & 68.3 & 91.0 \\ % no consistecy, no obj tok
            \rowspace
            {MViTv2 pretrain}             & 68.1 & 90.6 \\ % "multi task" pretrain
            \midrule
            % {{\model} - Different domains}     & -  & - 
            \rowspace
            % \vspace{0.38cm}
            {{\model}}                      & 68.9  & 91.3 \\ % Running
            \bottomrule
    %\label{tab:ssv2_ar}
\end{tabularx}

% \renewcommand*{\thefootnote}{\fnsymbol{footnote}}
% \begin{tabularx}
% {0.9\linewidth}{@{}l c c c c r@{}}
%     \toprule
%     {Model} & Boxes & Pretrain & {Top-1} & {Top-5}\\ 
%     \midrule
%     % SlowFast, R50 & \xmark & K400 & 61.7 & 87.0 & 65.7$\times$3$\times$1 & 34.1 \\
%     SlowFast, R101 & \xmark & K400 & 63.1 & 87.6  \\
%     TimeSformer-L & \xmark & IN & 62.5 & - \\
%     ViViT-L & \xmark & {\scriptsize IN+K400}  & 65.4 & 89.8 \\
%     MViT-B, 64 & \xmark & K600  &  68.7 &  91.5 \\

%     \midrule
    

%     \midrule
    

%     \bottomrule
% \end{tabularx}



==> Tables/Results/ssv2_part_notop5.tex <==
\renewcommand*{\thefootnote}{\fnsymbol{footnote}}
% \newcommand{\rowspace}{\vspace{0.075cm}}
\newcommand{\rowspace}{}

\begin{tabularx}
{1\linewidth}{@{}l l l c}
            \toprule
            & Model & {Top-1}  \\
            & & & \\
            \midrule
            & SlowFast, R101\methodwithoutboxes        & 63.1   \\
            \rowspace
            % TimeSformer-L               & 62.5  \\
            & ViViT-L     \methodwithoutboxes          & 65.4 \\
            \rowspace
            & MViTv1 \methodwithoutboxes & 64.7 \\
            % 16 $\times$ 4     &  64.7  \\
            \rowspace
            & MViTv2 \methodwithoutboxes & 68.1 \\
            % 16 $\times$ 4     &  68.1  \\
            \midrule
            & {MViTv2 MT} & 68.3 \\ % no consistecy, no obj tok
            \rowspace
            \midrule
            % {{\model} - Different domains}     & -  & - 
            \rowspace
            % \vspace{0.38cm}
            & {\modelPT} & 68.1\bcol{$\sim$0.0}  \\ % "multi task" pretrain
            & {{\modelDD}} & 68.2\gcol{$+$0.1}  \\ % Running
            & {{\modelID}}  & 68.9\gcol{$+$0.8}  \\ % Running
            \bottomrule
    %\label{tab:ssv2_ar}
\end{tabularx}

% \renewcommand*{\thefootnote}{\fnsymbol{footnote}}
% \begin{tabularx}
% {0.9\linewidth}{@{}l c c c c r@{}}
%     \toprule
%     {Model} & Boxes & Pretrain & {Top-1} & {Top-5}\\ 
%     \midrule
%     % SlowFast, R50 & \xmark & K400 & 61.7 & 87.0 & 65.7$\times$3$\times$1 & 34.1 \\
%     SlowFast, R101 & \xmark & K400 & 63.1 & 87.6  \\
%     TimeSformer-L & \xmark & IN & 62.5 & - \\
%     ViViT-L & \xmark & {\scriptsize IN+K400}  & 65.4 & 89.8 \\
%     MViT-B, 64 & \xmark & K600  &  68.7 &  91.5 \\

%     \midrule
    

%     \midrule
    

%     \bottomrule
% \end{tabularx}



==> Tables/ego4d_augs.tex <==
\begin{table*}
% 	\small
% 	\centering
% 	\tablestyle{10.5pt}{1.15}
% 	\begin{tabular}{l | c | c | c | c | l@{} | l@{} }
	\begin{tabular}{l  c  c  c  c}
            \toprule
             Model & Rand & Temporal & Spatial  & Val Temporal  \\
                   & Aug. & Views    & Views    & loc. error    \\
            \midrule
            {\model} & \xmark & 1 & 1 & 0.515 \\
            {\model} & \cmark & 1 & 1 &   \\
            {\model} & \cmark & 1 & 3 &  \\
            {{\model}} & \cmark & 3 & 3 &  \\
            \bottomrule
	\end{tabular}
    \caption{\textbf{Results on Ego4D PNR Temporal Localization.}}
	\label{tab:ego4d}
% 	\vspace{-1.0em}
\end{table*}

